AIMS.au: A Dataset for the Analysis of Modern Slavery Countermeasures in Corporate Statements

Despite over a decade of legislative efforts to address modern slavery in the supply chains of large corporations, the effectiveness of government oversight remains hampered by the challenge of scrutinizing thousands of statements annually. While Large Language Models (LLMs) can be considered a well established solution for the automatic analysis and summarization of documents, recognizing concrete modern slavery countermeasures taken by companies and differentiating those from vague claims remains a challenging task. To help evaluate and fine-tune LLMs for the assessment of corporate statements, we introduce a dataset composed of 5,731 modern slavery statements taken from the Australian Modern Slavery Register and annotated at the sentence level. This paper details the construction steps for the dataset that include the careful design of annotation specifications, the selection and preprocessing of statements, and the creation of high-quality annotation subsets for effective model evaluations. To demonstrate our dataset's utility, we propose a machine learning methodology for the detection of sentences relevant to mandatory reporting requirements set by the Australian Modern Slavery Act. We then follow this methodology to benchmark modern language models under zero-shot and supervised learning settings.

==> Laws_Table_reviewed_1811.tex <==
\begin{document}

\section{Comparison of Modern Slavery Reporting Criteria and Metrics}

\begin{landscape}
\begin{table}
\centering
\caption{Comparison of Modern Slavery Reporting Criteria and Metrics}
\vspace{0.1mm}
\fontsize{7}{7}\selectfont
\label{tab:appendix:examples}
%\begin{adjustbox}{width=\textwidth,height=\textheight} 
\begin{adjustbox}{scale=0.93}
    \begin{tabularx}{26cm}{|X|X|X|X|X|}
    \hline  % horizontal line at the top
         \textbf{AIMS.au Dataset Annotation Specification Questions} & \textbf{Australian Modern Slavery Act Mandatory Reporting Criteria} & \textbf{UK Modern Slavery Act Reporting Suggestions} & \textbf{Canadian Fighting Against Forced Labour and Child Labour in Supply Chains Act Reporting Obligations} & \textbf{The "Beyond Compliance" Walk Free \& WikiRate Metrics} \\
    \hline  % horizontal line after header

      \textcolor{darkgreen}{  Question: Is the statement approved by the entity's principal governing body?} & \textcolor{darkgreen}{Ensure that the statement is approved by the board.} & \textcolor{darkgreen}{Approval from the board of directors (or equivalent management body)} & \textcolor{darkgreen}{Approval by the organization’s governing body.} & \textcolor{darkgreen}{MSA Statement Approval: Was the company’s Modern Slavery Act statement explicitly approved by the board of directors (or equivalent management body)?} \\
    \hline

         \textcolor{darkgreen}{Question: Is the statement signed by a responsible member of the reporting entity?} & \textcolor{darkgreen}{The statement is signed by a responsible member of the organization. }&\textcolor{darkgreen}{ Signature from a director (or equivalent) or designated member }&\textcolor{darkgreen}{ Signature of one or more members of the governing body of each entity that approved the report.} & \textcolor{darkgreen}{MSA Statement Signed: Was the company’s Modern Slavery Act statement signed by an appropriate person?} \\
    \hline

        \textcolor{darkgreen}{ Question: Does the statement clearly identify which entities covered by the statement are the relevant reporting entities?}  & \textcolor{darkgreen}{Mandatory Criterion 1: The statement clearly identifies the Reporting Entity.} & \textcolor{darkred}{N/A} & \textcolor{darkred}{N/A } & \textcolor{darkred}{N/A} \\
    \hline

         \textcolor{darkgreen}{Question: Does the reporting entity describe its structure? \newline Question: Does the reporting entity describe its operations? \newline Question: Does the reporting entity describe its supply chains?} & \textcolor{darkgreen}{Mandatory Criterion 2: Describe the reporting entity’s structure, operations, and supply chains.} & \textcolor{darkgreen}{The organisation’s structure, business and supply chains.} & \textcolor{darkgreen}{Description of the organisation’s structure, activities and supply chains.} & \textcolor{darkgreen}{ MSA Organizational structure and operations: Does the company disclose the ownership structure(s) and/or business model(s) of each of its brands, subsidiaries, and other businesses covered by their Modern Slavery statement? \newline MSA Supply Chain Disclosure: Does the company’s statement identify the suppliers in their supply chain and/or the geographic regions where their supply chain operates? }\\
   \hline

         \textcolor{darkgreen}{Question: Does the reporting entity describe its modern slavery risks?} & \textcolor{darkgreen}{Mandatory Criterion 3: Describe the risks of modern slavery practices in the operations and supply chains of the reporting entity and any entities the reporting entity owns or controls.} & \textcolor{darkgreen}{Risk assessment and management.} & \textcolor{darkgreen}{Description of the parts of its business and supply chains that carry a risk of forced labour or child labour being used and the steps it has taken to assess and manage that risk.} & \textcolor{darkgreen}{MSA Identification of Risks?} \\
    \hline

         \textcolor{darkgreen}{Question: Does the reporting entity describe the actions applied to identify, assess, and mitigate the modern slavery risks it identified?} & \textcolor{darkgreen}{ Mandatory Criterion 4: Describe the actions taken by the reporting entity and any entities it owns or controls to assess and address these risks, including due diligence and remediation processes.} & \textcolor{darkorange}{ Description of the organisation’s policies in relation to slavery and human trafficking. \newline Description of the organisation’s due diligence processes in relation to slavery and human trafficking in its business and supply chains. \newline Description of the parts of the organisation’s business and supply chains where there is a risk of slavery and human trafficking taking place, and the steps it has taken to assess and manage that risk. \newline The training and capacity building about slavery and human trafficking available to its staff.} & \textcolor{darkorange}{  Description of the organisation’s policies and due diligence processes in relation to forced labour and child labour. \newline Description of the parts of organisation’s activities and supply chains that carry a risk of forced labour or child labour being used and the steps it has taken to assess and manage that risk. \newline The training provided to employees on forced labour and child labour.} & \textcolor{darkorange}{ MSA Policy (Revised): Does the company’s statement detail specific, organisational policies or actions to combat slavery in their direct (tier one) and/or in-direct (beyond tier one) supply chain? \newline MSA Risk assessment: How does the company assess the risks of modern slavery and trafficking in their supply chain? \newline MSA Risk management: Does the company continuously monitor suppliers to ensure that they comply with the company’s policies and local laws? \newline MSA Whistleblowing Mechanism (revised): Does the company have a grievance mechanism in place to facilitate whistleblowing or the reporting of suspected incidents of slavery or trafficking? \newline MSA Training (revised): Does the statement describe training for staff that is specifically geared towards detecting signs of slavery or trafficking?} \\
    \hline

         \textcolor{darkgreen}{ Question: Does the reporting entity describe remediation actions for modern slavery cases?} & \textcolor{darkgreen}{ Mandatory Criterion 4: Describe the actions taken by the reporting entity and any entities it owns or controls to assess and address these risks, including due diligence and remediation processes.}& \textcolor{darkgreen}{The organisation should paint a detailed picture of all the steps it has taken to address and remedy modern slavery, and the effectiveness of all such steps.} & \textcolor{darkgreen}{Description of any measures taken to remediate any forced labour or child labour.} & \textcolor{darkgreen}{MSA Incidents Remediation (revised): Did the company explain the corrective steps it has taken (or would take) in response to modern slavery incidents in their own operations and/or supply chain?} \\
    \hline

         \textcolor{darkgreen}{Question: Does the reporting entity describe how it assesses the effectiveness of its actions?} & \textcolor{darkgreen}{Mandatory Criterion 5: Describe how the reporting entity assesses the effectiveness of these actions.} & \textcolor{darkgreen}{Description of the organisation’s effectiveness in ensuring that slavery and human trafficking is not taking place in its business or supply chains, measured against such performance indicators as it considers appropriate. \newline The organisation should paint a detailed picture of all the steps it has taken to address and remedy modern slavery, and the effectiveness of all such steps. }& \textcolor{darkgreen}{ Description of how the entity assesses its effectiveness in ensuring that forced labour and child labour are not being used in its business and supply chains.} & \textcolor{darkgreen}{MSA Performance Indicators: Does the company define performance indicators that measure the effectiveness of their actions to combat slavery and trafficking?} \\
    \hline

         \textcolor{darkgreen}{Question: Does the reporting entity describe how it consulted on its statement with any entities it owns or controls? } & \textcolor{darkgreen}{Mandatory Criterion 6: Describe the process of consultation with any entities the reporting entity owns or controls.} & \textcolor{darkred}{N/A} & \textcolor{darkred}{N/A} & \textcolor{darkred}{N/A} \\
    \hline

         \textcolor{darkred}{N/A} & \textcolor{darkred}{Mandatory Criterion 7: Provide any other relevant information.} & \textcolor{darkred}{N/A} & \textcolor{darkred}{Any measures taken to remediate the loss of income to the most vulnerable families that results from any measure taken to eliminate the use of forced labour or child labour in its activities and supply chains.} & \textcolor{darkred}{MSA Impact on Company Behaviour: Does the company’s statement describe a change in their policy that occurred as a direct result of the Australian Modern Slavery Act? \newline MSA Business Performance Indicators: Has the company reviewed business KPIs to ensure they are not increasing risk of modern slavery? \newline MSA Historic Record: Does the company provide a historic record of their modern slavery statements (either on their website or in their current statement)?} \\
    \hline  % horizontal line at the bottom
    \end{tabularx}
\end{adjustbox}
\end{table}
\end{landscape}

\end{document}


==> results.tex <==
\section{Benchmark Experiments}
\label{sec:experiments}

In this section, we outline our experimental setup and present the results of benchmarking various models for detecting sentences relevant to the mandatory reporting requirements of the Act. We evaluate the performance of these models under both zero-shot and fine-tuning settings to assess their effectiveness in extracting mandated information from statements. We then analyze the results to identify key insights and potential areas for improvement.  % , and strategies for the future development of models that determine whether companies are meeting the requirements of modern slavery legislation  THIS LAST PART IS KEPT FOR THE CONCLUSION

\textbf{Task definition.} Our proposed dataset includes a variety of labels that models could predict; these labels are detailed in \appendixDatasetLabels{}. For conciseness and clarity, we focus on a task that we believe will be of greatest interest to the machine learning community: predicting relevant or irrelevant labels according to our eleven questions. We frame this task as a sentence-level binary classification problem which we evaluate across the eleven questions using F1, Precision, and Recall metrics. We selected these metrics over accuracy because they allow us to identify cases where models simply learn to predict all sentences as irrelevant, since those are over-represented in our dataset (see Figure~\ref{fig:data:annotation_stats:relevant_ratios}). %For experiments based on multiple criteria, we also provide Macro aggregation scores so that all criteria contribute the same to the final score.

For the statements that are double annotated by hired workers, we adopt a ``union'' label combination strategy, where a sentence is considered relevant if any annotator marks it as such. This approach addresses the possibility that individual annotators may have missed relevant text in some statements. We suggest that future works explore more sophisticated methods for leveraging annotator disagreements as a supervision signal. For our current experiments, models are evaluated exclusively using the subsets of ``gold'' annotated statements. Since these gold sets contain high-quality annotations, their smaller size (roughly 7000 sentences each) with respect to the overall dataset size should not significantly impact the reliability of model evaluations. Furthermore, this approach helps us, as well as future researchers, avoid incurring significant API usage costs when using state-of-the-art, closed-source language models for large-scale evaluations. % on a subset of statements annotated by external workers.

\textbf{Evaluated models.} We conduct our experiments using a range of language models that includes three open models --- DistilBERT~\cite{sanh2020distilbert}, BERT~\cite{devlin2019bert} and \llama{}~\cite{touvron2023llama} --- and two closed models, namely OpenAI's \gptthree{} and \gptfour{} (see \appendixImplDetails{} for more details). We use the OpenAI and \llama{} models to evaluate zero-shot (prompt-based) approaches, and we compare them with DistilBERT, BERT, and \llama{} models trained directly on statements annotated by hired workers. Our experiments are structured based on two input data setups: in the first (\emph{no-context} setup), models only have access to the target sentence being classified; in the second (\emph{with-context} setup), we provide additional context by including up to 100 words balanced before and after the target sentence (see \appendixPromptDesign{} for an example). This dual input setup allows us to assess the impact of contextual information on model performance. We also evaluate models based on two criteria setups: models either predict labels across all of our Mandatory Criteria questions, or only for the question related to supply chains (which is part of Criteria~2). This latter setup is representative of the dataset in terms of average difficulty, and is used due to the limitations of our current OpenAI API usage tier which prevents us from running large-scale experiments across all questions with \gptthree{} and \gptfour{} in time for submission. Note that we plan on completing these experiments following the submission of this preprint.

The ``open'' models (DistilBERT, BERT, and \llama{}) are fine-tuned from self-supervised pre-training checkpoints available on the HuggingFace repository~\cite{wolf2019huggingface}. For DistilBERT and BERT, we fine-tune the full model weights, while for \llama{}, we use the LoRA approach~\cite{hu2021lora} to manage computation costs. All experiments are conducted on a A100 GPU with 40~GB memory using PyTorch. Token sequence lengths are capped at 512 for DistilBERT and BERT, and at 150 for \llama{}, due to memory limitations. Models are trained with a batch size of 96 for DistilBERT, 64 for BERT, and 32 for \llama{}, using Adam~\cite{kingma2014adam} with a fixed learning rate (0.00003). We select model checkpoints that maximize the Macro F1-score across all criteria or the C2 (``supply chains'') F1-score for the single-question setup. Links to the model pages and checkpoint names are provided in \appendixImplDetails{}.

\textbf{Prompt design for zero-shot experiments.} Experiments with \gptthree{} and \gptfour{} are conducted using a prompt template designed specifically for C2 (``supply chains'') and given in \appendixPromptDesign{}. This template was designed following best practices on how to formulate intents, how to provide domain definitions, and how to constrain desired outputs~\cite{ekin2023prompt}. The definitions provided in the prompt are taken from the Act and its guidance document~\cite{amsa2018_legislation, amsa2018_guidance2023}, and are essentially a condensed version of the instructions given to the annotators. We leave the exploration of more sophisticated prompts, or very large prompts that may include multiple examples or even our entire annotation specifications document, for future works.

\subsection{Results}

\begin{table}[t]
    \centering
    \caption{Single-question evaluation results (for \ctwo{}), with and without context.}
    \vspace{2mm}
    \label{tab:experiments:results:c2supplychains}
    \begin{tabular}{lcccccc}
        %\toprule
        \multirow{2}{*}[-1mm]{\textbf{Model}} & \multicolumn{3}{c}{\textbf{No context}} & \multicolumn{3}{c}{\textbf{With context}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
                     & F1    & Precision & Recall & F1    & Precision & Recall \\
        \midrule
        DistilBERT   & 0.727 & 0.731     & 0.724  & 0.763 & 0.806     & 0.724 \\
        BERT         & 0.743 & 0.718     & 0.770  & 0.773 & 0.851     & 0.709 \\
        \llama{}     & 0.737 & 0.808     & 0.678  & -     & -         & -     \\
        \midrule
        \gptthree{}  & 0.317 & 0.195     & 0.837  & 0.174 & 0.096     & 0.996 \\
        \gptfour{}   & 0.543 & 0.464     & 0.656  & 0.556 & 0.412     & 0.852 \\
        %\bottomrule
    \end{tabular}
\end{table}

Table~\ref{tab:experiments:results:c2supplychains} presents the evaluation results for the single-question (C2, ``supply chains'') setting, both with and without context. Note that \llama{} results are unavailable with context due to computational constraints, as the longer input sequence would necessitate substantial token truncation. Across both the \emph{no-context} and \emph{with-context} setups, fine-tuned models consistently outperform zero-shot approaches, with the performance gap between these two model families being substantial.
%According to the LMSYS leaderboard~\cite{chiang2024chatbot} as of May 2024, \gptfour{} is the top-performing language model across various tasks. While its technical details are undisclosed, we can infer that \gptfour{} is considerably more complex than BERT or \llama{}. Here, \gptfour{} narrows the performance gap with fine-tuned models and outperforms \gptthree{}.
The fine-tuned models exhibit comparable performance, though there remains room for improvement. Precision and recall are generally balanced, except for \gptthree{}, which appears to classify nearly all sentences as relevant. Comparing results with and without context, we observe performance improvements for all models except \gptthree{}, possibly due to input sequence length exceeding the model's limitations. Future research should explore techniques to prepare or leverage context more effectively.
\begin{figure}[t]
\begin{center}
\vspace{2mm}
\includegraphics[width=\textwidth]{figures/results__all_labels.pdf}
\caption{F1 scores obtained by fine-tuned models trained jointly on the eleven relevant content questions, along with their overall (``Macro'') F1 performance. See \appendixAddResults{} for detailed results.}
\label{fig:experiments:results:all}
\end{center}
\end{figure}
We present evaluation results for all fine-tuned models on the full eleven-question setting in Figure~\ref{fig:experiments:results:all}, with detailed results in Appendix~\ref{sec:appendix:add_results}. We note again that zero-shot models are not presented here because each question requires a separate prompt, and in consequence the total number of requests to \gptthree{} or \gptfour{} exceeds the limits of our current OpenAI API usage tier. We note that the result trends are similar as in the previous \ctwo{} case, where tested models performed similarly, with \llama{} being slightly behind BERT and DistilBERT. We observe again, in general, that models provided with context outperform the no-context ones. Interestingly, results are visibly worse for \llama{} on the questions related to Criteria~5 (``effectiveness'') and~6 (``consultation''). We attribute this to the use of a suboptimal fine-tuning optimization strategy, chosen due to computational budget constraints, combined with the challenges posed by these two criteria, particularly the inherent difficulty of identifying their relevant text.



One final insight we emphasize is that, based on the presented results and our preliminary prompt engineering experiences, it is challenging to find prompts for zero-shot models that can match the performance of fine-tuned models.
%This contrasts strongly with the \emph{seemingly} straightforward nature of the task: determining whether a single sentence contains a relevant disclosure.
This highlights the necessity for high-quality, curated datasets like \dataset{} to allow for the reliable training and evaluation of language models. Additionally, this underscores the need for further exploration into the importance of context at various scales and the impact of vague and distracting text on large language models.

